Neural LerPlane Representations for Fast 4D Reconstruction of Deformable Tissues

Reconstructing deformable tissues from endoscopic stereo videos in robotic surgery is crucial for various clinical applications. However, existing methods relying only on implicit representations are computationally expensive and require dozens of hours, which limits further practical applications. To address this challenge, we introduce LerPlane, a novel method for fast and accurate reconstruction of surgical scenes under a single-viewpoint setting. LerPlane treats surgical procedures as 4D volumes and factorizes them into explicit 2D planes of static and dynamic fields, leading to a compact memory footprint and significantly accelerated optimization. The efficient factorization is accomplished by fusing features obtained through linear interpolation of each plane and enables using lightweight neural networks to model surgical scenes. Besides, LerPlane shares static fields, significantly reducing the workload of dynamic tissue modeling. We also propose a novel sample scheme to boost optimization and improve performance in regions with tool occlusion and large motions. Experiments on DaVinci robotic surgery videos demonstrate that LerPlane accelerates optimization by over 100$\times$ while maintaining high quality across various non-rigid deformations, showing significant promise for future intraoperative surgery applications.

==> 05_acknowledgements.tex <==
\subsubsection{Data Use Declaration and Acknowledgment.} 
% Authors must declare the data origin, data license, and (when appropriate) ethics application number for any public or private data used in the preparation of the paper.
This paper uses the EndoNeRF dataset, which is supported by Multi-Scale Medical Robotics Centre InnoHK, CUHK Shun Hing Institute of Advanced Engineering, and Shenzhen-HK Collaborative Development Zone. 

==> 06_supplyment.tex <==
\begin{figure}[htbp]
\includegraphics[width=\textwidth]{figs/tool_occlusion}
\caption{We present the ground truth, LerPlane results, and the difference map from left to right.
The results demonstrate the efficacy of our LerPlane approach in reconstructing deformable tissues and removing instruments. Specifically, following a mere 10 minutes of optimization, our LerPlane method delivers sound and high-quality tissue reconstruction, implying the enormous potential for intraoperative use. Note that regions persistently occluded by instruments might not be optimally restored due to the limited information available for these areas. Please zoom in for more details.
} \label{fig: overview}
\end{figure}

==> 07_bib.tex <==
\begin{thebibliography}{8}
\bibitem{endonerf}
Wang, Y., Long, Y., Fan, S. \& Dou, Q. Neural Rendering for Stereo 3D Reconstruction of Deformable Tissues in Robotic Surgery. {\em MICCAI (8)}. \textbf{13437} pp. 431-441 (2022)

\bibitem{edssr}
Long, Y., Li, Z., Yee, C., Ng, C., Taylor, R., Unberath, M. \& Dou, Q. E-DSSR: Efficient Dynamic Surgical Scene Reconstruction with Transformer-Based Stereoscopic Depth Perception. {\em MICCAI (4)}. \textbf{12904} pp. 415-425 (2021)

\end{thebibliography}

==> tables/aba.tex <==
\begin{tabular}{c|cccc}
\hline
Methods   & PSNR           & SSIM          & LPIPS         & FLIP           \\ \hline
Ours-NS   & 29.831 ± 2.208 & 0.925 ± 0.020 & 0.081 ± 0.022 & 0.1 ± 0.1\\
Ours\_TS  & 29.831 ± 2.208 & 0.925 ± 0.020 & 0.081 ± 0.022 & 0.1 ± 0.1\\
Ours\_VE  & 29.831 ± 2.208 & 0.925 ± 0.020 & 0.081 ± 0.022 & 0.1 ± 0.1\\
Ours\_NE  & 29.831 ± 2.208 & 0.925 ± 0.020 & 0.081 ± 0.022 & 0.1 ± 0.1\\ \hline
\end{tabular}

==> tables/table_minipage.tex <==
\begin{table}[t]
\scriptsize
\begin{minipage}[b]{0.555\linewidth}
 %\fontsize{9pt}{1.5}\selectfont
 %\tabcolsep=0.25cm
 
	\begin{center}
	\caption{Ablation Study on the masking teacher assistant (MTA), on ACDC test set under 7 labeled cases settings. (DSC{[}\%{]}/ASD{[}mm{]}).}
  \label{ab_MTA}
	\vspace{-3pt}
	\label{table:acdc_lits_main}
       %\begin{adjustbox}{width=0.95\linewidth}
	\begin{tabular}{cccc|cc}
		\toprule
       &Teacher & Student & MTA & DSC~$\uparrow$ & ASD~$\downarrow$ \\ \midrule
\multirow{5}{*}{\makecell[c]{Mask \\ ratio}}   & 0.0 &    0.6 & N/A & 87.08 & 0.76 \\ 
 & 0.0 &    0.4 & 0.2 & 87.86 & 0.67 \\         
&     0.0 &    0.6 & 0.3 & \textbf{88.21} & \textbf{0.46}\\
&     0.0 &   0.8 & 0.4 & 88.15 & 0.49\\
 &  0.0 &    0.99 & 0.5 & 86.61 & 0.62\\ 

		              \bottomrule        
	\end{tabular}
    %\end{adjustbox}
    \end{center}
\end{minipage}
\begin{minipage}[b]{0.42\linewidth}
	\begin{center}
	\caption{Ablation Study of different strong perturbation methods, on ACDC test set under 7 labeled cases settings. (DSC{[}\%{]}/ASD{[}mm{]}).}
 \label{ab_perb}
	\vspace{-3pt}
	\label{table:acdc_lits_main}
       %\begin{adjustbox}{width=0.95\linewidth}
	\begin{tabular}{c|cc}
		\toprule
        Perturbation & DSC~$\uparrow$ & ASD~$\downarrow$ \\ \midrule
         w/o   & 82.42 & 1.10 \\         
           Gaussian Blur & 83.93 & 1.08\\
            Colorjitter &  81.76& 2.05\\
            Mask & \textbf{86.61}& \textbf{0.62}\\
	\bottomrule        
	\end{tabular}
    %\end{adjustbox}
    \end{center}
\end{minipage}
    %\vspace{-20pt}
    
\end{table}  

==> tables/tables.tex <==
\begin{tabular}{c|cccc|c}
\hline
Methods  & PSNR$\uparrow $        & SSIM$\uparrow$         & LPIPS$\downarrow$         & FLIP$\downarrow$            & Time$\downarrow$            \\ \hline
E-DSSR   & 13.398{\tiny $\pm$}1.387   & 0.630 {\tiny $\pm$}0.057  & 0.423 {\tiny $\pm$}0.047  & \textbackslash{} & \textbackslash{} \\
EndoNeRF & 29.272{\tiny $\pm$}2.836   & 0.921 {\tiny $\pm$}0.022  & 0.088 {\tiny $\pm$}0.020  & 0.085{\tiny $\pm$}0.018    & 14 $h$             \\ \hline
Ours-NS  & 31.532{\tiny $\pm$}1.665   & 0.886{\tiny $\pm$}0.021   & 0.142 {\tiny $\pm$}0.020  & 0.112{\tiny $\pm$}0.016      & 3 $min$            \\
Ours-TS  & 31.544{\tiny $\pm$}1.669   & 0.886{\tiny $\pm$}0.021   & 0.142{\tiny $\pm$}0.020   & 0.111{\tiny $\pm$}0.015      & 3 $min$            \\
Ours-VE  & 32.353{\tiny $\pm$}1.742   & 0.897{\tiny $\pm$}0.022   & 0.131{\tiny $\pm$}0.024   & 0.103{\tiny $\pm$}0.012      & 3 $min$            \\
Ours-NE  & 32.230{\tiny $\pm$}1.655   & 0.895{\tiny $\pm$}0.023   & 0.131{\tiny $\pm$}0.020   & 0.102{\tiny $\pm$}0.012      & 3 $min$            \\
% Ours-NW  & 31.908{\tiny $\pm$}1.521   & 0.889{\tiny $\pm$}0.023   & 0.137{\tiny $\pm$}0.027   & 0.108{\tiny $\pm$}0.013      & 3 $min$            \\ 
\hline
Ours-9k  & 32.589{\tiny $\pm$}1.451   & 0.901{\tiny $\pm$}0.021  & 0.126{\tiny $\pm$}0.028    & 0.103{\tiny $\pm$}0.014      & 3 $min$            \\
Ours-32k & 35.504{\tiny $\pm$}3.076   & 0.935{\tiny $\pm$}0.026  & 0.083{\tiny $\pm$}0.022    & 0.075{\tiny $\pm$}0.031    & 10 $min$           \\ \hline
\end{tabular}

